A New Framework for Centrality Measures in Multiplex Networks

The non-trivial structure of such complex systems makes the analysis of their collective behavior a challenge. The problem is even more difficult when the information is distributed across networks (e.g., communication networks in different media); in this case, it becomes impossible to have a complete, or even partial picture, if situations are analyzed separately within each network due to sparsity. A multiplex network is well-suited to model the complexity of this kind of systems by preserving the semantics associated with each network. Centrality measures are fundamental for the identification of key players, but existing approaches are typically designed to capture a predefined aspect of the system, ignoring or merging the semantics of the individual layers.

==> framework.tex <==
%!TEX root = ./Multi-HITS.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Framework
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalization}
\note{define what a configuration is.}


\begin{center}
\begin{figure}[h!]
  \begin{subfigure}[b]{.31\linewidth}
    $A_0 A_0^T A_1 A_1^T$  
    \caption{}
    \label{fig:conf0}
  \end{subfigure}
  \hspace*{\fill}
    \begin{subfigure}[b]{.31\linewidth}    
      $A_0  A_1 A_0^T A_1^T$   
    \caption{}
    \label{fig:conf1}
  \end{subfigure}
  \hspace*{\fill}
    \begin{subfigure}[b]{.31\linewidth}    
      $A_0  A_1^T A_0^T A_1  $  
    \caption{}
    \label{fig:conf2}
  \end{subfigure}
  
     \begin{subfigure}[b]{.31\linewidth}
    $A_0 A_0^T A_1^T A_1 $  
    \caption{}
    \label{fig:conf0}
  \end{subfigure}
  \hspace*{\fill}
    \begin{subfigure}[b]{.31\linewidth}    
      $A_0  A_1 A_1^T A_0^T $   
    \caption{}
    \label{fig:conf1}
  \end{subfigure}
  \hspace*{\fill}
    \begin{subfigure}[b]{.31\linewidth}    
      $A_0  A_1^T A_1 A_0^T   $  
    \caption{}
    \label{fig:conf2}
  \end{subfigure}
  
    \caption{All possible configurations for a multiplex network of two layers}
    \label{fig:all_conf}
\end{figure}
\end{center}


%% MULTIPLEX
\begin{figure}[h]
\centering
\input{multiplex-img.tex}
\caption{Multiplex Network with $\mathcal{L}$ layers}
    \label{fig:frmwGraph}
\end{figure}


%% CONFIGURATIONS FORMULAE
The number of all the possible \textit{configuration} is:
\begin{equation}
 \sum_{k=1}^{2\ell} \binom{2\ell}{k} (k-1)! 
\end{equation}


%% RANKINGS DEPENDENCIES
\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A)[minimum size=0.6cm] at (4.5,2.5) {$r_0$};
    \node (B)[minimum size=0.6cm] at (7.5,2.5) {$r_1$};
    \node (C)[minimum size=0.6cm] at (7.5,0) {$r_2$};
    \node (D)[minimum size=0.6cm] at (4.5,0) {$r_3$}; 
    \node[draw=none] at (6,-1.2) {$(c)$};
 \end{scope}

\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (B) edge[bend right=0] node {$A_0^T$} (A);
    \path [->] (C) edge[bend right=0] node {$A_0$} (B);
    \path [->] (D) edge[bend right=0] node {$A_1^T$} (C);
    \path [->] (A) edge[bend right=0] node {$A_1$} (D);
    \end{scope}



\begin{scope}[every node/.style={circle,thick,draw}]
    \node (E)[minimum size=0.6cm] at (0,0) {$a$};
    \node (F)[minimum size=0.6cm] at (3,0) {$h$};
     \node[draw=none] at (1.5,-1.2) {$(b)$};
    \end{scope}
\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (F) edge[bend right=30] node {$A_0^T$} (E);
    \path [->] (E) edge[bend right=30] node {$A_0$} (F);    
\end{scope}


\begin{scope}[every node/.style={circle,thick,draw}]
    \node (G)[minimum size=0.6cm] at (1.5,2.5) {$p_r$};
     \node[draw=none] at (1.5,1.6) {$(a)$};
      \end{scope}
\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (G) edge[out=30,in=100,looseness=6] node {$G$} (G);   
\end{scope}

\end{tikzpicture}
\caption{Formulation of PageRank (a), HITS (b) and Multiplex HITS-Like (c) rankings in \MRF Framework}
    \label{fig:frmwGraph1}
\end{figure}


==> ring-img.tex <==
%!TEX root = ./Multi-HITS.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ring in a Multiplex Network
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[scale=0.45,on grid]
		
	

	\begin{scope}[
		yshift=-25,xshift=5,
		every node/.append style={yslant=\yslant,xslant=\xslant},
		yslant=\yslant,xslant=\xslant	]	
		
		\fill[white,fill opacity=.75] (1.1,1.2) rectangle (6.8,5.8); 
		\draw[black, dashed, thin] (1.1,1.2) rectangle (6.8,5.8);  
			
		\draw[fill=black,opacity=0.4, thick]  						
			(2,3.5) node(111){} circle (.1)
			(3,5.232050808) circle (.1)
			(5,5.232050808) circle (.1)
			(6,3.5) circle (.1)			
			(5,1.767949192)  circle (.1)
			(3,1.767949192)  circle (.1);
									
						
			\draw[-latex, thin]
			(2,3.5) to (3,5.232050808)	;	
			\draw[-latex, thin]
			(5,5.232050808) to (6,3.5);
			\draw[-latex, thin]
			(5,1.767949192) to (3,1.767949192);
		
		\fill[black]
			(0,6.0) node[above, scale=.7] {\textbf{Layer 1}}	
			(0,5.5) node[above, scale=.7] {\textbf{(} $A_1$, $A_1^T$ \textbf{)} }		
			(1.5,3.5)  node[right,scale=.7]{\bf 2}
			(2.5,5.232050808)  node[right,scale=.7]{\bf 3}
			(5,5.232050808) node[right,scale=.7]{\bf 4}
			(6,3.5)   node[right,scale=.7]{\bf 5}			
			(5,1.767949192) node[right,scale=.7]{\bf 6}
			(2.5,1.767949192)  node[right,scale=.7]{\bf 1};		

	\end{scope}
	
	
	
		
	% Interlayer crossconnections
	%\draw[black, dotted, thick, decoration={ segment length=1mm, amplitude=0.6mm},opacity=1] (-3.8,1.1) to (-3.8, 2.25);
	%\draw[black, dotted, thick, decoration={ segment length=1mm, amplitude=0.6mm},opacity=1] (-3.8,2.7) to (-3.8, 3.8);
	%\draw[black, dotted, thick, decoration={ segment length=1mm, amplitude=0.6mm},opacity=1] (-3.8,4.3) to (-3.8, 5);
	%\draw[black, dotted, thick, decoration={ segment length=1mm, amplitude=0.6mm},opacity=0.65] (-4.45,1) to (-4.45, 2.55);
	%\draw[black, dotted, thick, decoration={ segment length=1mm, amplitude=0.6mm},opacity=0.65] (-4.45,2.85) to (-4.45, 4.2);
	
	
	% Layer 0
	\begin{scope}[
		yshift=0,
		every node/.append style={yslant=\yslant,xslant=\xslant},
		yslant=\yslant,xslant=\xslant
	]
		\fill[white,fill opacity=.55] (1.1,1.2) rectangle (6.8,5.8); 
		\draw[black, dashed, thin] (1.1,1.2) rectangle (6.8,5.8);  
			
		\draw[fill=black,opacity=0.4, thick]  	
					
			(2,3.5) node(111){} circle (.1)
			(3,5.232050808) circle (.1)
			(5,5.232050808) circle (.1)
			(6,3.5) circle (.1)
			(3,1.767949192)  circle (.1)
			(5,1.767949192)  circle (.1);
			
			\draw[-latex, thin]
			(3,1.767949192) to (2,3.5)	;	
			\draw[-latex, thin]
			(6,3.5) to (5,1.767949192);
			\draw[-latex, thin]
			(3,5.232050808) to (5,5.232050808);
	
		
		\fill[black]
			(0,6.0) node[above, scale=.7] {\textbf{Layer 0}}	
			(0,5.5) node[above, scale=.7] {\textbf{(} $A_0$, $A_0^T$ \textbf{)} }		
			(1.5,3.5)  node[right,scale=.7]{\bf 2}
			(2.5,5.232050808)  node[right,scale=.7]{\bf 3}
			(5,5.232050808) node[right,scale=.7]{\bf 4}
			(6,3.5)   node[right,scale=.7]{\bf 5}			
			(5,1.767949192) node[right,scale=.7]{\bf 6}
			(2.5,1.767949192)  node[right,scale=.7]{\bf 1};			
	\end{scope} 
\end{tikzpicture}

==> sec_intro.tex <==
%!TEX root = ./Multi-HITS.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}

Networks provide a powerful representation of interaction patterns in complex systems. \cite{1,2,3}
The structure of social relations among individuals, interactions between proteins, food webs, and many other situations can be represented using networks.
Until recently, the vast majority of studies in network science have focused networks that consist of a single type of entity, with different entities connected to each other via a single type of connection. 
Such networks are now called single-layer (or monolayer) networks. The idea of incorporating additional information -- such as multiple types of interactions, subsystems, and time-dependence -- has long been pointed out in various fields, such as sociology \cite{4, 5} and engineering \cite{6}, but an effective unified framework for the mathematical treatment of such multidimensional structures, which are usually called multilayer networks, has been developed only recently \cite{7, 8}.
Multilayer networks can be used to model many complex systems. For example, relationships between humans include different kinds of interactions -- such as relationships between family members, friends, and coworkers -- that constitute different layers of a social system. Different
layers of connectivity also arise naturally in natural and human-made systems in transportation \cite{9}, ecology\cite{10}, neuroscience\cite{11}, and numerous other areas. The potential of multilayer networks for representing complex systems more accurately than was previously possible has led to an explosion \cite{2} of work on the physics of multilayer networks.
The main question posed a few years ago concerned the implications of multilayer structures for the dynamics of complex systems, and several seminal papers about interdependent networks -- a special type of multilayer network -- revealed that such structures can change the qualitative behaviors in a significant way \cite{12, 13}.
These findings thus posed the challenge for how to account for multiple layers of connectivity in a consistent mathematical way. 
An explosion of recent papers has developed the field of multilayer networks into its modern form, and there is now a suitable mathematical framework\cite{14} and novel structural descriptors\cite{15,16,17,18,19} for studying these systems.
Many studies have also started to highlight the importance of analyzing multilayer networks, instead of relying on their monolayer counterparts \cite{20, 21}, 
to gain new insights about empirical systems.
Nowadays, we know that the study of multilayer networks is fundamental for enhancing our understanding of dynamical processes on real networked systems,
such as flow (or its congestion) in transportation network \cite{22, 23}, cascading failures in interdependent infrastructures\cite{12}, and information
and disease spreading in social networks\cite{24,25,26,27}. For instance, when two spreading process are coupled in a multilayer network, 
the onset of one disease-spreading process depends on the onset of the other one, yielding a curve of critical points in the phase diagram of the parameters that govern a system's spreading dynamics\cite{25}. Such a curve reveals the existence of two distinct regimes, such that the criticality of the two dynamics may or may not be interdependent.
Similarly, cooperative behavior can be enhanced by multilayer structures, providing a novel way for cooperation to survive in structured populations\cite{28}.
For additional examples, see various reviews and surveys\cite{7, 8, 13, 24, 29,30,31} on multilayer networks and specific topics within them.
A multilayer framework allows a natural representation of coupled structures and coupled dynamical processes. 
Here, after a brief overview on the representation of multilayer networks, we will focus on dynamical processes in which multilayer analysis has revealed new physical behavior. 
Specifically, we will discuss two cases: (i) a single dynamical process, such as continuous and discrete diffusion, running on the top of a multilayer structure; and (ii) different dynamical processes, each one running on the top of each layer and coupled/mixed by a multilayer structure.

\subsection{HITS}
Kleinberg's HITS (Hyperlink-Induced Topic Search) algorithm (Kleinberg 1999) is a link analysis algorithm which was originally developed in a Web context; HITS is thought to be useful for inferring Web pages that would be considered authorities for a particular query made to a search engine. This deduction uses only the information from the structure of a directed graph built on the basis of the particular query, and which is a subgraph of the directed graph representing the Web. The algorithm selects some nodes of this directed graph through the exploitation of a mutual reinforcing relationship. Recent applications of the HITS algorithm in fields far removed from that of Web searching, such as that of word stemming (Bacchin, Ferro and Melucci 2002), and the discovery of a connection between the technique of HITS and the Latent Semantic Indexing technique (Ng et al. 2001), have led us towards a theoretical study of this algorithm. In fact we think that an in-depth mathematical analysis is necessary to better understand the behaviour of this algorithm in various contexts. The purpose of this analysis is that of deriving properties to decide if the algorithm could reasonably be applied in other fields.
In this paper we perform this mathematical analysis, considering a general formulation of the algorithm from which the original algorithm can be deduced as a particular case; we focus on the convergence of the algorithm and on the study of its symmetry. We have tried to carry out this analysis examining the algorithm independently of its Web application, so that we address some aspects of the algorithm that are crucial to having a wider knowledge of its general behaviour.
The analysis of retrieval algorithms in general is not yet typical in Information Retrieval. A technical survey on Information Retrieval on the Web can be found in Agosti and Melucci (2001) and Henzinger (2001) is a brief survey focused on hyperlink analysis for the Web. Kleinberg's original work is described in Kleinberg (1999). The cited article introduces the HITS algorithm in a Web context; HITS is used to rank the Web pages retrieved by a text- based search engine in response to a specific query. Since Kleinberg's algorithm works on a subgraph built on the basis of the query, it is said to be an algorithm which gives a query- dependent ranking, as opposed to the algorithms giving a query-independent ranking, such as PageRank (Page et al. 1998), used by the Google search engine (Brin and Page 1998). SALSA, another famous link analysis algorithm for performing query-dependent ranking, is described in Lempel and Moran (2001). These and other link analysis algorithms are studied in depth in Borodin et al. (2001), where some useful criteria to compare link analysis algorithms are also defined. The stability of link analysis algorithms, i.e. how much these algorithms are perturbed by the changing of a portion of the set of Web pages on which they are working, is studied in Ng et al. (2001). We have been led towards the mathematical analysis of the HITS algorithm described here by the results presented in Bacchin, Ferro and Melucci (2002). This latter work uses the core of Kleinberg's algorithm in a context far removed from that of Web searching, that is the context of word stemming. In Ng et al. (2001) there is another interesting application of the algorithm in a different context, the one of traditional Information Retrieval for "flat" documents; in the cited paper there is an attempt to see the connections between HITS and the well-known Latent Semantic Indexing technique. A brief theoretical analysis of the HITS algorithm to study its limitations in a Web context is performed in Miller et al. (2001); this analysis is used to suggest new algorithms that try to overcome these limitations.
This paper is structured as follows. In Section 2 we give some mathematical results that should be remembered in order to understand the progression of the paper. Section 3 sets out Kleinberg's algorithm and the generalization of the algorithm we are considering here. Sections 4 and 5 study the convergence of the algorithm. Section 6 studies the symmetry of the algorithm and proves the equivalence between symmetry and the order of the basic update operations. Since this work has a theoretical aim, we do not give a list of all its possible applications. In Section 7, however, we expound some interesting consequences of our theoretical results.

==> trash.exp.tex <==

We focused especially on the HITS-Like configuration, verifying that is the natural generalization of HITS. We used two different models of random graphs: the Erdos-renyi model and the Stochastic Block Model (SBM) introduced in Chapter \ref{chap:2} and illustrated in Figure \ref{fig:graph_types}. \\
The first one was conceived to underline the similarity of our method to HITS. The second one is oriented on checking the differences between the differences between the configurations of the same equivalence class. The last two experiments are based on the convergence. We studied the convergence of the algorithm when varying the parameters

\item The first experiment show which are the differences of score obtained by an HITS like method formulated with \OUR and the scores obtained by using the original HITS %(and PageRank) 
formulation over each layer of the multiplex network.
We are going to build a synthetic multiplex network obtained applying the following steps:
\begin{itemize}
\item the first step consists of the generation of a graph $G(V,E)$ according to one of the selected topology (Random graph, Erdos-Renyi, Barabasi-Albert, Watts-Strogatz, Exponential random (ERGM), Hyperbolic (HGN), Hierarchical, Stochastic block model);
\item the second step assign, according to a given probability $p$, each edge of $G$ to one or more layer of the multiplex network $M$.\\
Let be ${p_0,...,p_\ell}$ the set $\PrL$ (each $p$ should be independent or sums to 1) of the probabilities assigned to each layer $ \ell \in L(M)$ then:\\
$$\forall_{e\in E},\quad\forall_{ \ell \in L(M)}: e\cup E_\ell \quad according \quad to \quad p_\ell$$
\end{itemize}
Measure the similarity between the obtained layers using the Jaccard coefficient over the edges. For each group of graphs ( grouped by size = $2^s, 6 \le s \le 10$ ), 
plot the relation between the Jaccard and  the weighted-tau obtained concatenating all rankings of each algorithm \textit{configuration}


%%%%% NOT PROCESSED %%%%%%



\begin{enumerate}



\item Show all the possible \textit{configuration} without repetition over a multiplex network of $\ell$ layer. 
To understand level of similarity between each \textit{configuration}, concatenate all rankings and finally compare them using the weighted-tau.
\item Study the speed of convergence to the stationary point based on $\tau$ and the generated network. 
\end{enumerate}



The experiment (2) was meant to show the differences between the different rankings related to the different equivalence classes. For this simulations we used the same type of generators as used in (1) but with a fixed size of the set of nodes: 256. Figures \ref{fig:exp3_erdos} and \ref{fig:exp3_sbm} show the values of weighted tau between the rankings related to the element of a fixed configuration and the members of the same equivalence class with the rankings obtained running the HITS algorithm on the configuration in the "normal form",i.e $A_0^TA_0A_1^TA_1$. In these plots we can see the "stratification" as well: the line at the top is the the same as in Figure \ref{fig:exp1_er} and \ref{fig:exp1_sbm}. The one just below that cuts across the plot is related to $A_1^TA_1A_0^TA_0$ and its behavior makes sense if we think that is referring to the network with inverted layers and how the weighted tau works. The difference between the line above, in terms of matrices, is that the last two matrices of $A_0^TA_0A_1^TA_1$ are now the first ones (multiplied in the same orders) and the first ones are now at the end (always multiplied in the same order). The result is that the position of the two transposes and the two matrices are exchanged. Comparing the two ranks we obtain a lower tau but it converges to 1 when the layers get similar becoming the same. Since to identical layers correspond identical matrices, when Jaccard equals 1, $A_0^T=A_1^T$ and $A_0=A_1$ so the concatenated vector is equal to the one obtained from the previous multiplication of the matrices, namely $A_0^TA_0A_1^TA_1$. The last two lines, lowest ones, derive from a multiplication where both indexes and transposes are inverted from $A_0^TA_0A_1^TA_1$. 



\begin{center}
\begin{figure}[h!]
  \begin{subfigure}[b]{0.48\linewidth}
  \includegraphics[width =\linewidth]{exp2/e2_erdos_config_A_0A_1_TA_1A_0_T.pdf}
  \caption{}\label{fig:exp3_erdos}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\linewidth}
  \includegraphics[width =\linewidth]{exp2/e2_sbm_config_A_0A_1_TA_1A_0_T.pdf}
  \caption{}\label{fig:exp3_sbm}
  \end{subfigure}
  \caption{Experiment 2: Weighted tau related to the equivalence class $A_0A_1^TA_1A_0^T$ using an Erdos-Renyi graph (a) and a Stochastic Block Model (b) as generator.}
  \label{fig:exp3_A0T_A0}
\end{figure}
\end{center}

\begin{center}
\begin{figure}[h!]
  \begin{subfigure}[b]{0.48\linewidth}
  \includegraphics[width =\linewidth]{exp2/e2_erdos_config_A_0A_1A_1_TA_0_T.pdf}
  \caption{}\label{fig:exp3_erdo}
  \end{subfigure}
  \begin{subfigure}[b]{0.48\linewidth}
  \includegraphics[width =\linewidth]{exp2/e2_sbm_config_A_0A_1A_0_TA_1_T.pdf}
  \caption{}\label{fig:exp3_sb}
  \end{subfigure}
  \caption{Weighted tau related to the equivalence class $A_0A_1^TA_1A_0^T$ using an Erdos-Renyi graph (a) and a Stochastic Block Model graph as generator (b).}
  \label{fig:exp3_A0_A1}
\end{figure}
\end{center}

The results seen for the second experiment in Figure \ref{fig:exp3_A0T_A0} were about the configuration of the HITS-Like method where the Hubs of one layer was influenced from the Authorities of the same level and the authorities was depending on the Hubs of the next layer and so on. This configuration is the same represented in in figure 2c. For a simpler understanding we will write this configuration as 

\begin{figure}
	\begin{tikzpicture}
    \begin{scope}[every node/.style={circle,thick,draw}]
    \node (A)[minimum size=0.6cm] at (1,2.5) {$h_0$};
    \node (B)[minimum size=0.6cm] at (3.5,2.5) {$a_0$};
    \node (C)[minimum size=0.6cm] at (6,2.5) {$h_1$};
    \node (D)[minimum size=0.6cm] at (8.5,2.5) {$a_1$}; 
    \node[draw=none] at (5,0.5) {$(a)$};
 \end{scope}

\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (B) edge[right] node {$A_0^T$} (A);
    \path [->] (C) edge[right] node {$A_0$} (B);
    \path [->] (D) edge[right] node {$A_1^T$} (C);
    \path [->] (A) edge[bend left] node {$A_1$} (D);
    \end{scope}
	
	\end{tikzpicture}
    \label{fig:confA_0^TA_0}
\end{figure}

We investigate also the configuration where all the Hubs are influenced by the Hubs of the successive layer and just the last one depends by the Authorities and the same rule stands  for the Authorities in order to close the cycle. This configuration is shown in Figure

\begin{figure}
	\begin{tikzpicture}
    \begin{scope}[every node/.style={circle,thick,draw}]
    \node (A)[minimum size=0.6cm] at (1,2.5) {$h_0$};
    \node (B)[minimum size=0.6cm] at (3.5,2.5) {$h_1$};
    \node (C)[minimum size=0.6cm] at (6,2.5) {$a_0$};
    \node (D)[minimum size=0.6cm] at (8.5,2.5) {$a_1$}; 
    \node[draw=none] at (5,0.5) {$(b)$};
 \end{scope}

\begin{scope}[>={Stealth[black]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (B) edge[right] node {$A_0^T$} (A);
    \path [->] (C) edge[right] node {$A_1^T$} (B);
    \path [->] (D) edge[right] node {$A_0$} (C);
    \path [->] (A) edge[bend left] node {$A_1$} (D);
    \end{scope}
	
	\end{tikzpicture}
    \label{fig:confA_0A_1}
\end{figure}




%%%%%%%%%%% ABSTARCT ORIG STI %%%%
Networks are presents in all aspect of our world and constitute the backbone of many services such as gas, electricity, and water. Networks permeate any kind of transportation systems (train, buses, air-flights, and naval). In the medical domain we find networks that model the complex interplay between phenotype and genotype. The most impressive scenario involve the human being at any level. Peoples, states and organizations, heavily interacts one with each other, using several types of media. We are deeply interconnected using severals social platforms (Facebook, Twitter, Instagram, etc.), telephone, short text and voice messages (e-Mail, Messenger, SMS, WhatsApp).

The properties of the collective behaviors and of their dynamics are deeply characterized by the non-trivial  structure of this real-world complex systems. The problem becomes more difficult if we consider that information is distributed across different networks and it is impossible to have a complete or partial picture, if individual situations are analyzed in isolation.

Using a multiplex network is the natural way to model this complex system and captures the complexity of the system without losing the semantics associated with each network.
Centrality measures is the most important measures to find the key players of our world. Several centrality measures have been proposed in the literature (PageRank, HITS, Versatile, etc.) over the last decades. Each centrality measure is focuses on analyzing a specific aspect of the system, ignoring or merging the semantics of the individual layers.

We present a Framework for Semantic Aware Centrality Measures in Multiplex networks (\MRF). 
\MRF Framework tackle all the outlined problems (sparsity and data distribution, mixed semantics, inflexibility of the measures) encompassing and generalizing the previous approaches. \MRF enables the encoding of specific dependencies between the subnets of Multiplex networks to  define semantic aware centrality measures.
We develop a theoretically sound iterative method based on Perron-Frobenius theory, and formally prove its convergence, to compute the rankings in conditions of highly sparsity and data distribution.

We massively investigate the behavior of our methodology defining a synthetics environment. Our methodology was compared  with existing techniques, and also theoretical complexity was analyzed. We study the influence of the chosen subnets of Multiplex networks, and we also test the convergence of our method.

The conducted extensive experiments clearly shown the power and flexibility of the proposed framework.


%%%%%%%%% RUNNINNG TIME %%%%%
\begin{table*}[ht]
  \centering
    \begin{adjustbox}{width=0.98\linewidth}
	\begin{tabular}{r r l r l r l r l r l r l}
    $\mathbf{|V|}$&\multicolumn{2}{c}{\textbf{PageRank}}&\multicolumn{2}{c}{\textbf{PageRank-Like}}&\multicolumn{2}{c}{\textbf{HITS}}&\multicolumn{2}{c}{\textbf{HITS-Like}}&\multicolumn{2}{c}{\textbf{Versatile}}&\multicolumn{2}{c}{\textbf{Versatile-Like}}\\
        \hline \hline
64	&	0.034 &$\pm$ 9.7e-4	&	0.177 &$\pm$2.3e-3	&	0.074 &$\pm$1.3e-3	&	0.454 &$\pm$4.6e-3	&	64.297 &$\pm$3.2e-1	&	0.223	&$\pm$	3.1e-3\\
128	&	0.132 &$\pm$3.9e-3	&	0.262 &$\pm$3.0e-3	&	0.234 &$\pm$6.3e-3	&	0.779 &$\pm$1.3e-2	&	257.654 &$\pm$1.2e+0 &	0.302	&$\pm$	3.8e-3\\
256	&	0.521 &$\pm$1.6e-2	&	0.736 &$\pm$8.9e-3	&	0.886 &$\pm$2.0e-2	&	3.034 &$\pm$4.0e-2	&	1027.000 &$\pm$5.0e+0&	0.729	&$\pm$	8.0e-3\\
512	&	2.310 &$\pm$7.6e-2	&	3.764 &$\pm$4.7e-2	&	3.424 &$\pm$7.4e-2	&	19.922 &$\pm$1.3e-1	&	3651.454 &$\pm$4.7e+1 &	3.038	&$\pm$	2.9e-2\\
1024&	11.014 &$\pm$3.2e-1	&	27.312 &$\pm$1.4e-1	&	12.027 &$\pm$2.5e-1	&	135.864 &$\pm$6.7e-1&	10489.905 &$\pm$1.8e+2 &	16.235&$\pm$	2.5e-1\\
     \hline \hline
  \end{tabular}
  \end{adjustbox}  
  \caption{Running time of the compared methods using an Erdos-Renyi graph as generator. \label{tab:complexity-erdos}}  
  
  \subsubsection{}
\end{table*}

\begin{table*}[ht]
  \centering
    \begin{adjustbox}{width=0.98\linewidth}
	\begin{tabular}{r r l r l r l r l r l r l}
    $\mathbf{|V|}$&\multicolumn{2}{c}{\textbf{PageRank}}&\multicolumn{2}{c}{\textbf{PageRank-Like}}&\multicolumn{2}{c}{\textbf{HITS}}&\multicolumn{2}{c}{\textbf{HITS-Like}}&\multicolumn{2}{c}{\textbf{Versatile}}&\multicolumn{2}{c}{\textbf{Versatile-Like}}\\
        \hline \hline
64	&	0.023 &$\pm$ 5.5e-4	&	0.183 &$\pm$2.5e-3	&	0.153 &$\pm$3.9e-3	&	0.450 &$\pm$4.6e-3	&	64.756 &$\pm$3.5e-1	&	0.230	&$\pm$	3.1e-3\\
128	&	0.074 &$\pm$2.1e-3	&	0.263 &$\pm$2.8e-3	&	0.593 &$\pm$2.0e-2	&	0.798 &$\pm$1.5e-2	&	257.481 &$\pm$1.3e+0 &	0.299	&$\pm$	3.5e-3\\
256	&	0.279 &$\pm$8.3e-3	&	0.745 &$\pm$8.2e-3	&	2.489 &$\pm$7.1e-2	&	2.963 &$\pm$3.9e-2	&	1028.674 &$\pm$4.9e+0&	0.714	&$\pm$	8.1e-3\\
512	&	1.042 &$\pm$3.4e-2	&	3.903 &$\pm$5.6e-2	&	10.745 &$\pm$2.9e-1	&	19.368 &$\pm$1.3e-1	&	3847.040 &$\pm$2.1e+1 &	3.149	&$\pm$	2.5e-2\\
1024&	3.995 &$\pm$1.1e-1	&	28.691 &$\pm$1.7e-1	&	43.141 &$\pm$1.1e+0	&	136.268 &$\pm$7.3e-1&	14529.359 &$\pm$2.1e+2 &20.824	&$\pm$	2.6e-1\\
     \hline \hline
  \end{tabular}
  \end{adjustbox}  
  \caption{Running time of the compared methods using an SBM graph as generator. \label{tab:complexity-SBM}}  
\end{table*}
